Too Afraid to Drive: Systematic Discovery of Semantic DoS Vulnerability in Autonomous Driving Planning under Physical-World Attacks

In high-level Autonomous Driving (AD) systems, behavioral planning is in charge of making high-level driving decisions such as cruising and stopping, and thus highly securitycritical. In this work, we perform the first systematic study of semantic security vulnerabilities specific to overly-conservative AD behavioral planning behaviors, i.e., those that can cause failed or significantly-degraded mission performance, which can be critical for AD services such as robo-taxi/delivery. We call them semantic Denial-of-Service (DoS) vulnerabilities, which we envision to be most generally exposed in practical AD systems due to the tendency for conservativeness to avoid safety incidents. To achieve high practicality and realism, we assume that the attacker can only introduce seemingly-benign external physical objects to the driving environment, e.g., off-road dumped cardboard boxes. To systematically discover such vulnerabilities, we design PlanFuzz, a novel dynamic testing approach that addresses various problem-specific design challenges. Specifically, we propose and identify planning invariants as novel testing oracles, and design new input generation to systematically enforce problemspecific constraints for attacker-introduced physical objects. We also design a novel behavioral planning vulnerability distance metric to effectively guide the discovery. We evaluate PlanFuzz on 3 planning implementations from practical open-source AD systems, and find that it can effectively discover 9 previouslyunknown semantic DoS vulnerabilities without false positives. We find all our new designs necessary, as without each design, statistically significant performance drops are generally observed. We further perform exploitation case studies using simulation and real-vehicle traces. We discuss root causes and potential fixes.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> ccs-body.tex <==
\section{Introduction}

This is a sample!  It does not have a lot of fancy stuff in it, but if
you want to see a more complex sample, look at the original ACM
templates.

To fill up enough text to fill up 3 pages, we've included the CCS Call
for Papers three times.  It is always a good idea to include some
gratuitious citations to recent CCS papers~\cite{medvinsky1993netcash,
  bellare1993random, anderson1993cryptosystems, blaze1993cryptographic}.

\input{cfp}
\input{cfp}
\input{cfp}

\section{Conclusions}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

\appendix

\section{Location}

Note that in the new ACM style, the Appendices come before the References.

\input{cfp}

\begin{acks}
% TODO: For the submission, don't include acknowledgments since they would most likely deanonymize you.
\end{acks}


==> summary_changes.tex <==
\twocolumn
[
\section*{\Large Revision Summary}
\vspace{0.2in}
]
\setcounter{subsection}{0}

%\subsection{Short Summary of Primary Changes}
%\todo{Finish the short sumnmary after finishing the detrailed ones.}

The first version of the paper was submitted to NDSS'22 Fall and received a Major Revision decision. We thank the reviewers for their constructive comments; as shown below, these comments substantially benefited this paper in various aspects, especially scientific rigor and clarity. In the following, we provide detailed point-by-point responses and revision descriptions (in \fbox{boxes}) to each of the revision requirements.

%in\newparts{~\S{}A}. After that, in\newparts{~\S{}B} we further describe our responses and revisions to several other issues raised in the individual reviews but not included in the major revision requirements.

\cut{
%Alfred: not necessary; this is required by oakland

This revised version has 3 primary changes:
\begin{itemize}
    \item \textbf{Tone down the overclaims.} We tone down our claims in introduction and challenges section to avoid misleading. We clearly define our contribution to show the novelty of our work without over claiming any contributions in prior works.
    
    \item \textbf{More comprehensive evaluation.} Following the suggestions from the reviewers, we collected diverse traces for each scenario to make our experiment more comprehensive. We also run the efficiency comparison with more scientific setup and commonly-used metrics to demonstrate the effectiveness and efficiency of our system design. 
    
    \item \textbf{More discussion about the exploitation and potential fixes.} We add more discussion for the discovered vulnerabilities as suggested by reviewers, including the root cause, vulnerability exploitation, and potential mitigations. 
\end{itemize}


%\subsection{Detailed Responses to List of Revision Requirements}
%\label{sec: mr-requirement}

In this section, we provide point-by-point responses to the list of revision requirements provided with the Major Revision decision. For each revision requirement, we first echo the corresponding original reviews for the convenience of the reviewers, and then provide our responses and corresponding paper revisions in \fbox{boxes}.
}

\textit{The paper was discussed extensively by the reviewers and additionally in the PC discussion meeting. The reviewers were interested in the techniques proposed by the authors, but a lack of clarity in the threat model and overclaimed contributions throughout the paper (particularly in the methodology and evaluation) made it impossible to fully endorse the work in its present form. We'd like to invite the authors to resubmit this paper after addressing the following major revisions:}

%Alfred: no need
%\begin{response}
%We thank the reviewers for their insightful and constructive feedback for improving the paper. We have addressed the clarity problem in Revision~\ref{rev:distinction},~\ref{rev:exploit},~\ref{rev:case_exploitation},~\ref{rev:evaluation_setup},~\ref{rev:test_goal},~\ref{rev:clarify_mitigation}.\end{response}

\textit{Provide a more thorough explanation of the threat model:}
\textit{(1) Explain the distinction between semantic (logic) bugs and traditional software bugs (e.g., memory corruption bugs).}

\begin{response}
Thanks a lot for suggesting such important clarification. We added a dedicated explanation for this, and also added a figure (Fig.~2). Basically, the semantic BP DoS vulnerability targeted in this paper is a type of semantic software vulnerability for BP, which can be caused by either software design flaws or implementation bugs. The key distinction of such semantic vulnerabilities to traditional software bugs is that their symptoms are erroneous behaviors at the BP decision logic level (e.g., keep driving or not, change lane or not) instead of at the generic computer program level (e.g., software crash, memory corruption, hang). In our problem setting, since we target physical-world attack vectors (\S\rom{2}-C), the semantic BP vulnerabilities we target further differ in that the vulnerability triggering is via physical-world realizable perturbations (e.g., by adding attacker-controllable road objects) instead of generic program input changes (e.g., bit-level value changes of BP inputs), which is also illustrated in Fig.~2.
%adding distinction between semantic (logic) bugs and traditional software bugs. Traditional software bugs have explicit erroneous program behavior, such as a crashor assertion failure. On the other hand, semantic bugs refer to the outputs of the program are unexpected and usually specifications are needed to detect such type of bugs. Specifically in our problem context, the semantic BP bugs mean that the generated planning trajectory is unexpected, which could be either overly-aggressive or overly-conservative.
\end{response}
\begin{revision}\label{rev:distinction}
We added a dedicated clarification under ``Distinction to traditional software bugs'' at the end of the attack goal section (\S\rom{2}-B) to explain the above, and also added Fig.~2 for better illustrations of such distinction.
%We compare the general (traditional) software vulnerability exploitation with semantic BP vulnerability exploitation in Fig.~2 and \S\rom{2}-C. We explain that how they are different in terms of failure pattern. 
\end{revision}

\textit{
(2) Clarify how semantics bugs are caused by design flaws (safety issues--naturally happens) and can be triggered by an adversary (security issues).}
\cut{
\begin{link}

\textbf{Corresponding original reviews:} 

Reviewer C:

\textit{The biggest concern I have is whether this is a security paper. All 9 cases shown in this paper are normal cases we may experience during driving. As these are normal cases. I don't think this belongs to security conference. I believe this paper fits much better to robotics conference such as ICRA or software engineering conference ICSE. I feel uncomfortable to see "attack scenario" and "DoS vulnerabilities". The bugs shown here are purely software bugs causing malfunctioning even without attackers. Therefore, I don't think this paper belongs to NDSS.}
\end{link}
}

\begin{response}
Thanks a lot for suggesting this, which is another important aspect that we need to clarify. We added a dedicated explanation for this. Under our physical-world attack threat model, the attack-targeted unintended BP decision behaviors are indeed also possible to naturally occur in non-adversarial settings, making them also in the scope of general safety or robustness problems. Here, we would like to clarify that the distinction is that we focus on the set of such unintended behaviors that are \textit{(more) triggerable} by attackers in the driving environment, e.g., easily-controllable road objects such as cardboard boxes, bikes, and attacker-driven vehicles, instead of weather conditions and road-side building locations/shapes. Note that such a security focus makes the discovered vulnerabilities  arguably more severe, since with an adversary such naturally-occurable unintended behaviors can be more frequently, controllably, and strategically triggered to cause more severe real-world consequences, e.g., causing emergency brakes in more dangerous road segments such as highway ramps, and causing traffic blocking in mission-critical roads such as in front of police stations or fire stations.

%We make the following clarifications in the revised paper: %\begin{itemize}
%\item Even though the DoS BP vulnerabilities can naturally happen, they are still triggerable by a valid threat model. We compare this pattern with tradition software fuzzing research and demonstrate that they are essentially the same: the attacker inject malicious inputs and cause corresponding attack consequences by exploiting the internal bugs or design flaws. 

%\item Even though the attacker can not directly compromise the inputs to BP directly, the attacker can still use controllable objects in physical world and affect the BP inputs to finally exploit the vulnerabilities.  
%\end{itemize}
\end{response}

\begin{revision}\label{rev:exploit}
We added a dedicated clarification under ``Distinction to safety problems'' at the end of the threat model section (\S\rom{2}-C) to clarify the distinction. 
\end{revision}


\textit{(3) Support the case studies and examples on how an adversary can exploit these bugs to force an AV to undesired states (e.g., stopping the vehicle).}
%\begin{link}
%\textbf{Corresponding original reviews:} 
%Reviewer C:
%\textit{The biggest concern I have is whether this is a security paper. All 9 cases shown in this paper are normal cases we may experience during driving. As these are normal cases. I don't think this belongs to security conference. I believe this paper fits much better to robotics conference such as ICRA or software engineering conference ICSE. I feel uncomfortable to see "attack scenario" and "DoS vulnerabilities". The bugs shown here are purely software bugs causing malfunctioning even without attackers. Therefore, I don't think this paper belongs to NDSS.}
%\end{link}

\begin{response}
We agree that we need to clarify more on how an attacker can concretely exploit the discovered vulnerabilities in the case studies and examples. We followed the suggestion in our revision, and here are some highlights:
\begin{itemize}
    \item For the vulnerability for \textit{Lane Following DoS Attack on Autoware} (\S\rom{6}-A): To exploit this vulnerability, the attacker can find a single-lane road that is up to 4.35m wide (applicable to both common local and highway roads~\cite{lane_width}), and put two easy-to-carry objects such as cardboard boxes on each side of the road. There is no strict relative longitudinal position requirement for them, as long as they are in the same planning range (35m for Autoware). Since Autoware uses a more conservative safety buffer size than Apollo, for a narrow road width such as 2.7m~\cite{lane_width}, each of such object can be $>$80cm to the road boundary to make them look more stealthy. An example setup in the simulator is shown in Fig.~4~(C). This can cause an emergency stop and/or permanent stop of the victim AD vehicle and thus damage the AD service, block traffic, and also potentially road safety (from emergency stop). 
    
    \item For the vulnerability for \textit{Intersection Passing DoS Attack on Apollo} (\S\rom{6}-B): To exploit this vulnerability, the attacker can find any stop sign-based intersections, and place road-side parked bikes as long as they are within 5m from the lane center of any lanes in the intersection (illustrated in Fig.~25). Here, 2 parked bicycles are enough to bypass all timeout mechanisms in Apollo BP (detailed in Appendix~D-G). This can then force the AD vehicles to stop in front of the stop line forever.
    
    \item For the vulnerability for \textit{Lane Changing DoS Attack on Apollo} (\S\rom{6}-C): To exploit this vulnerability, for lanes with $\leq$3.55m width (applicable to almost all common local and highway lanes (up to 3.6m wide)~\cite{lane_width}), the attacker just needs to drive a normal-size car (e.g., 2.11m as in~\S\rom{3}-A) to follow a victim AD vehicle with close following distance (up to 8m). This can then prevent the AD vehicle from making lane changes forever, which can make it fail to arrive at the destination (especially critical for AD services such as robo-taxi/delivery). For lanes wider than 3.55m, the attacker just needs to drive with a slight deviation to the lane center (e.g., 5cm for a 3.6m-wide lane, which is far from touching the lane line ($>$70cm)) towards the direction she want to prevent the victim from changing lane to.
\end{itemize}
%We concretize the concept of triggering objects controllable by attacks in Revision 2 in each case study and example to show how an adversary can exploit those bugs. 
\end{response}
\begin{revision}\label{rev:case_exploitation}
We added a dedicated clarification under ``Exploitation method'' in each case study sections (\S\rom{6}-A, \S\rom{6}-B, \S\rom{6}-C) to detail how an adversary can exploit the vulnerability to force a victim AD vehicle to undesired states (e.g., stop vehicle, emergency brake, give up lane changing).
%We add more details in the Exploitation setup subsections for each case study in \S\rom{6}. 
\end{revision}

\textit{Reviewers require the following revisions for the Evaluation and Case Studies:}

\textit{(1) Provide a more thorough and clear description of the evaluation setup, including the perception errors, valid values for test inputs, and differences between Apollo and Autoware behavioral planning algorithms.}
\cut{
\begin{link}
\textbf{Corresponding original reviews:} 

Reviewer B:
 
\textit{Additionally, it is not clear whether the weather conditions and vehicle speeds impact the vulnerabilities. This analysis is required to understand the root cause of each vulnerability. For instance, how do you ensure that any of the vulnerabilities are not due to the sun reflection that impacts the boundary of the object? or how do you ensure the vehicle speed is not smaller than an amount (e.g., 10mph) that never will happen on the road?}

Reviewer E:

\textit{In general, scenarios like parked bicycles mistaken for pedestrians at a crosswalk seem more likely a sensor problem and probably can be solved by improving the software.}

\end{link}
}
\begin{response}
Thanks for suggesting adding these important evaluation setup details. We followed the suggestion in our revision, and here are some highlights:
\begin{itemize}
    \item On \textit{perception error}: Since we directly inject the attack objects at the planning input level using their ground-truth physical properties (e.g., type, bounding-box size and shape), we can avoid finding violation cases due to perception errors (e.g., caused by sun reflection).
    \item On \textit{valid values for test inputs}: For each attack object, BPFuzz initializes and mutates their properties within common feasible ranges according to their types. For example, the positions of generated objects is within 80m to the ego vehicle (a common range of AD perception~\cite{teslasensorcoverage}); the sizes for static objects are 0.5-2m in each dimension, and those for pedestrians and vehicles are the same as the default ones used in the simulator. We put all details into Table~\rom{6} in Appendix. Consistent with our threat model (\S\rom{2}-C), we do not mutate the non-attacker-controllable planning inputs such as weather condition and ego vehicle driving speed; all of them just inherit the valid values from original input traces (e.g., at the road speed limit for ego vehicle speed).
    \item On \textit{differences between Apollo and Autoware behavioral planning algorithms}: Their main difference is that Autoware's BP adopts a single finite state machine-based design where all planning behavior changes are modeled as state transitions, while Apollo's is more modular, which first decomposes the whole driving decision making into independent primitive tasks (e.g., obstacle avoidance, lane changing, intersection passing, velocity selection, etc.) and then selects the appropriate ones based on different driving scenarios (e.g., lane following, intersection, stop sign).
\end{itemize}






%We admit that details are missing in current version. We add more details, including evaluation setup, hardware, valid values of test inputs and difference between Apollo and Autoware behavioral planning algorithm. For the perception errors, since we assume that the other AD system components are perfect and thus there is no perception error in design. We will clarify this in the paper.
%We agree with the reviewers that our previous description is not clear and may lead to confusion. We clarify that there is \textit{no perceptional error} in our evaluation when testing behavioral planning since we directly generate the object detection and prediction results as part of planning input. For \textit{valid values of test inputs}, we explain how we mutate the input in valid ranges to ensure that the overly-conservative planning behavior is not caused by other reasons other than design flaws or bugs in BP. For the difference between Apollo and Autoware, we explain the different high-level design choices. Also, Apollo and Autoware have different concrete implementation, we want to clarify that there is no direct relationship between vulnerabilities in Apollo and vulnerabilities in Autoware.
\end{response}

\begin{revision}\label{rev:evaluation_setup}
We created dedicated descriptions under ``Test input generation'' in \S\rom{5}-A to provide the above details on perception error and valid values for test inputs. The details on the differences between Apollo and Autoware behavioral planning algorithms are added to the end of \S\rom{5}-A ``Subject BP implementations''.
\end{revision}


\textit{(2) Conduct new experiments to include more traces per scenario (as stated in the rebuttal response).}
\cut{
\begin{link}
\textbf{Corresponding original reviews:} 

Reviewer B:

\textit{Unfortunately, 15 traces collected under 8 different driving scenarios do not provide details on the vehicles and the environment it operates.  }

Reviewer C:

\textit{In evaluation, only 15 traces are used. It is a small number to ensure the generality of the vulnerabilities. As a fuzzing paper, you should show its coverage. Finally, "Evaluating Fuzz Testing" paper [87] shows requirement for fuzzing paper. Authors are recommended to follow requirements from that paper.}
\end{link}
}

\begin{response}
We agree that the number and diversity of collected traces is limited in previous version. We collected much more driving traces, resulting in 5 per scenario and 40 in total, which is \textit{more than doubled} compared to the previous version) and lead to 2.41$\times$ more initial testing seeds used in the evaluation. These traces have high diversity in terms of different type of roads (e.g., 2.7m, 3m, and 3.5m, ranging from minimal width in local road and common highway lane width), different driving tasks (e.g., driving straight, left turn, right turn), and different road structures (e.g., four-way intersection, three-way intersection). These does not lead to the discovery of new unique vulnerabilities though, which shows that the vulnerabilities discovered in our previous version have a certain degree of generality to different road type, driving tasks, and road structure.
\end{response}
\begin{revision}\label{rev:trace_collection}
We have collected new traces to reach 40 evaluated traces in total under 8 different driving scenarios (5 per scenario). We described this updated setup in the last paragraph of \S\rom{5}-A ``BP input trace collection''. Details of each of these 40 traces are provided in Table~\rom{5} in Appendix.
\end{revision}

\vspace{0.15cm}
\textit{
(3) Provide new evaluation metrics for the discovered vulnerabilities, such as the number of unique discovered vulnerabilities and time-to-exposure for the vulnerabilities.}
\cut{
\begin{link}
\textbf{Corresponding original reviews:} 

Reviewer C:

\textit{As a fuzzing paper, you should show its coverage. Finally, "Evaluating Fuzz Testing" paper [87] shows requirement for fuzzing paper. Authors are recommended to follow requirements from that paper.}


Reviewer E:

\textit{The evaluation is the main weakness of the paper. It does neither show the performance of BPFuzz nor does not it provide comparison to alternative approaches. BPFuzz starts with arbitrary scenarios. BPFuzz is run ten times until a problematic scenario was found. Then, a modified BPFuzz with reduced feature set was run. Given the same number of executions, the performance drops. I think this is not a reasonable strategy to evaluate the performance of a fuzzer.}


\textit{For a solid evaluation, fuzzers should be run for a defined time. All findings of the fuzzer in this period should be reported. Otherwise, a fair evaluation is not ensured. For example, if an alternative fuzzer would find the same bugs later (say 5 minutes later), then this would not be shown in this evaluation. The run-time of BPFuzz (between 1 and 235s, on average 53s) is too short for a sound fuzzer evaluation; typically a run-time of 24h is advised. I'd like to see some performance numbers which compare the effectiveness of the analysis phase and the simulation phase. How long do simulations take? What hardware was used?}

\textit{In the evaluation in Table 3, only the average was taken to indicate the runtime. In general, the arithmetic average is a difficult metric as it can hide many properties, e.g., a high variability. For example, in such scenarios it can hide variance between runs, e.g., variances in number of executions and run-time. For more information on fuzzer evaluation, I suggest the following paper: Klees, George, et al. "Evaluating fuzz testing." Proceedings of the 2018 ACM SIGSAC Conference on Computer and Communications Security. 2018.}

\end{link}
}
\begin{response}
Thanks a lot for suggesting such more rigorous evaluation methodology. We followed the suggestion to improve our baseline evaluation (\S\rom{5}-C) by (1) running each of the baseline setups and the full BPFuzz setup on the same testing seed for \textit{10 times}, each time for \textit{24 hours}, to avoid variance as suggested by Reviewer E and the ``Evaluating fuzz testing'' paper~\cite{klees2018evaluating}; (2) for each setup, we measure the \textit{discovered unique vulnerabilities} (defined in~\S\ref{subsec:evaluation_setup}) and also their \textit{average Time-to-Exposure ($\mu$TTE)}, i.e., the time taken to discover them; and (3) When comparing a given baseline setup with the full BPFuzz, we use \textit{statistical testing} following the suggestions in prior works~\cite{arcuri2011practical, klees2018evaluating, bohme2017directed}. Specifically, we use the \textit{Vargha-Delaney statistic $\Hat{A}_{12}$} to measure the effect size, and use \textit{Mann-Whitney U}~\cite{arcuri2011practical} to measure the statistical significance of the $\mu$TTE performance drop, which is the recommended measure for comparing randomized algorithms like fuzzers~\cite{arcuri2011practical, bohme2017directed}.

Table~\ref{tab:ablation_study} shows the results using these new evaluation metrics. For clarity, we denote the baseline setup that excludes only our BP vulnerability distance design (\S\ref{subsec:vuln_dist}) as \textit{BPFuzz}$^{-\textrm{\textit{guide}}}$; the setup that excludes only our PI-aware physical-object generation (\S\ref{subsec:design_mutation}) as \textit{BPFuzz}$^{-\textrm{\textit{PI}}}$; and the setup that excludes both as \textit{PB-M}, which directly use Protobuf-mutator (a directly-compatible traditional fuzzer) for the entire test input generation process. More details on these baseline setups are in~\S\ref{subsec:evaluation_ablation} ``Baseline setups''.

As shown in the table, PB-M, the setup without using any of our main problem-specific designs, fails to detect \textit{any} of the 9 BP DoS vulnerabilities within 24h (last column in Table~\ref{tab:ablation_study}), which is thus at least $57\times$ less efficient/effective. This concretely shows that our main problem-specific designs, BP vulnerability distance and PI-aware physical-object generation, are \textit{necessary} for effectively discovering BP DoS vulnerabilities. We further find that each of these two design components are also important when evaluated individually: for almost all (7/9) vulnerabilities, the $\mu$TTE performance drops are \textit{statistically significant} for both BPFuzz$^{-\textrm{guide}}$ and BPFuzz$^{-\textrm{PI}}$ (bold $\Hat{A}_{12}$ values in Table~\ref{tab:ablation_study}). From the $\mu$TTE values, BPFuzz$^{-\textrm{guide}}$ and BPFuzz$^{-\textrm{PI}}$ are on average \textit{$>$4.5$\times$} and \textit{$>$3.5$\times$} slower respectively; for complicated cases such as V1, such degradation can be even \textit{over 7$\times$} for BPFuzz$^{-\textrm{guide}}$. More discussions are in~\S\ref{subsec:evaluation_ablation}.


%We would like to thank the reviewers for the suggestions. We include following changes in the revised version: (1) We give a defined runtime (24h suggested by Reviewer-E) for each setup. (2) We report number of discovered vulnerabilities and TTE to compare the effectiveness and efficiency of each setup. (3) Following the suggestion in the paper pointed out by Reviewer-E~\cite{klees2018evaluating}, we report the statistical significance of performance via U-test and the effect size $\Hat{A}_{12}$ to address the concern of variance raised by Reviewer-E. 
%Our results show that by enabling the data flow distance, we can at least 24\% of vulnerability discovery time when the vulnerability takes more than 50 seconds to be discovered without data flow distance. The guidance can lead to 1.95-7.74$\times$ speed up on most of (7/9) the cases. All the aforementioned results are supported with significant statistical difference. When removing all the domain-specific input generation and mutation operations, the traditional syntax-based fuzzing tool could not find the vulnerabilities in the given time.


%We don't directly follow reviewer-C's suggestion to show coverage since this is not a general fuzzing work. Our goal is to discover vulnerabilities that can reach a specific program position. So we follow the approach in similar work~\cite{bohme2017directed} and use Time-to-Exposure (TTE) to compare the testing effectiveness. 
\end{response}

\begin{revision}\label{rev:evaluation_metric}
In our baseline evaluation in \S\ref{subsec:evaluation_ablation}, we adopt the new evaluation setup (each setup 10 times, each time for 24 hours) and new evaluation metrics for the discovered vulnerabilities (the number of unique discovered vulnerabilities and time-to-exposure for the vulnerabilities), which is described in \S\ref{subsec:evaluation_ablation} ``Evaluation setup and metrics''. The evaluation results are all updated according to these setups and metrics. We also updated related sentences throughout the paper (e.g., in abstract, introduction, and conclusion)
%We re-run the efficiency evaluation with the suggested metrics (e.g., time-to-exposure, the number of discovered vulnerabilities in 24h) and the new results are included in \S\rom{5}-C.
\end{revision}

\textit{
The issues below similarly need better documentation among other concerns noted by individual reviews; these include:}

\textit{(1) Clarify whether you are looking for cases that represent the bugs in the BP code or a set of scenarios that an adversary triggers a specific bug by placing physical objects.}
\cut{
\begin{link}
\textbf{Corresponding original reviews:}

Reviewer B:

\textit{After reading the decision logic of behavior planning algorithms (Figure 2), the root cause of the DoS attacks introduced in the paper is due to the fact that the BP algorithms apply overly conservative decisions (lateral buffer (0.4m) for the detected objects) while computing the driving space. Here I fail to understand whether the goal of the BPFuzz is to find this particular bug or to find scenarios that trigger this bug in AD behavioral planning algorithms. If the paper claims to achieve the latter, the paper might give some concrete cases (positioning of different objects considering the vehicle size and environment it is operating) that cause the bugs, which might be a better approach than reporting a set of scenarios as vulnerabilities.}
\end{link}
}

\begin{response}
We are looking for previously-unknown semantic DoS vulnerabilities at the BP code level, not the scenarios that trigger those (but a concrete scenario that triggers them will come with the discovery since it is a dynamic testing). Here each vulnerability we aim to discover has unique code-level decision logic (branches) that causes such vulnerability (e.g., those identified in~\S\ref{subsec:mov_example}), which is similar to unique crashes in popular fuzzers\cite{afl, yun2018qsym, chen2018angora, stephens2016driller}. Such unique vulnerable code logic for V1-V9 are documented under ``Vulnerable code'' in each section in Appendix.D.

So back to the reviewer's major revision question, our design goal is more towards the former (``looking for cases that represent the bugs in the BP code''), but we would like to emphasize that the vulnerabilities we are looking for are \textit{previously-unknown}; this is thus why \textit{their discoveries must happen first} before a systematic identification of their triggering scenarios is possible. Since our target is program-based BP due to their general adoption in today’s industry-grade AD systems (\S\ref{subsec:background_bp}), discovering such vulnerable code logic is already (and generally more) useful for AD developers in identifying root causes and potential code-level fixes (e.g., patches) compared to a comprehensive set of triggering scenarios; one concrete triggering scenario that comes with the discovery in our dynamic testing is already enough to understand the triggerability of a discovered vulnerability. 

%Our focus is exactly the former (``looking for cases that represent the bugs in the BP code''), not the scenarios that trigger those (but a concrete scenario that triggers them will come with the discovery since it is a dynamic testing).

%The focus of BPFuzz is to find previously-unknown semantic DoS vulnerabilities at the BP code level, not the scenarios that trigger those (but a concrete scenario that triggers them will come with the discovery since it is a dynamic testing). 
%Our goal is to find a concrete input that leads to an overly conservative driving behavior of behavioral planning. This is the same as normal fuzzing works. The popular fuzzing work “Evaluating Fuzz Testing” defined the goal of fuzzing as generating an input that causes the program to crash. Back to the reviewer’s question, we aim to find a particular bug by generating an input that leads to overly conservative driving behavior. BPFuzz is not aware of the existence of the vulnerabilities before the testing.
\end{response}
\begin{revision}\label{rev:test_goal}
We added a dedicated clarification of the above under ``Design goal'' at the very beginning of the BPFuzz design section (\S\rom{4}).
%We also clarify the BPFuzz outputs in the end of ``System input/output and assumptions'' in \S\rom{4}-B.
%We clarify the goal of BPFuzz and emphasize that we are not aware of the existence of vulnerabilities before testing in the first paragraph of \S\rom{4}. We also add clarification of the system inputs and outputs in the first paragraph of \S\rom{4}-B.
\end{revision}
\textit{
(2) Address all unintentional false claims and overclaims highlighted by the reviewers.}
%\redtodo{Change the challenges and related works section to avoid over cliams.}

\begin{link}
To ensure that we addressed all the unintentional false claimed pointed out by the reviewers, we first echo the related original reviews: 

Reviewer D:

\textit{However, the authors dismiss previous work and tend to overclaim the importance of the problem and its contributions. The authors also have several claims that are false. For example, on page 6, the authors say:}

\textit{The testing process cannot obtain any guidance on which test inputs are closer to triggering the vulnerability... So far, existing testing methods for semantic vulnerabilities/bugs in AD systems either do not consider obtaining such feedback (i.e., black-box testing) [92] or require the algorithm under test to be differentiable}

\textit{This is simply not true. Tools for falsification of CPS have long used quantitative feedback to guide search; even 10 years ago, tools like S-TaLiRo and Breach obtained "such feedback," and the techniques have improved in the decade since.}

\textit{Furthermore, the abstract states the following:}

\textit{Prior works on AD systems security concentrate on semantic vulnerabilities caused by environmental sensing errors, leaving those specific to such key decision-making processes an open problem.}

\textit{This is again not true. For example, paper [83] found more failures to behavior prediction and planning problems than perception failures (see Table IV).}

\textit{The paper also mentions several times issues about dealing with complex geometric constraints, generating scenarios subject to conditions, etc., and how no previous work has focused on this. Again, this is a bit misleading because there are tools specifically to enable what the authors claim is nonexistent. E.g.,}

\textit{Fremont, Daniel J., et al. "Scenic: a language for scenario specification and scene generation." Proceedings of the 40th ACM SIGPLAN Conference on Programming Language Design and Implementation. 2019.}

\textit{In general, the paper is written in a way that minimizes previous work and exaggerates the problem and contributions of the authors. Right now, we are designing autonomous driving software in a conservative manner to minimize safety problems, and the results of this research might not be a problem once developers start expanding the envelope on what is safe and become less conservative.}

Reviewer B:

\textit{It is not clear from Figure 1 [63] the reason makes the car got stuck in the middle of the road and how authors are sure that this is due to Waymo's behavior planning algorithm as motivated in Figure 3. The authors would consider providing more evidence for this motivating example.}

\end{link}
\begin{response}
Thanks a lot for pointing out all these overclaims. We fully agree that we need to tone down our claims in these descriptions. We followed the suggestion in our revision, and here are some highlights:
\begin{itemize}
    \item About \textit{quantitative feedback}: We clearly acknowledged that in the general CPS testing domain, prior works have used quantitative feedback such as the robustness metrics to guide testing~\cite{hekmatnejad2020search, kimpgfuzz}. We also clarified that such a guidance still treats the code-level decision logic (i.e., decision-making code branches) as black-box, which thus cannot provide guidance once the overall planning output stays unchanged. In our problem setting, it is desired if we can improve this with more fine-grained code-level guidance such as the distance between the current inputs and the planning decision boundary at the code branch level. For example, in Fig.~\ref{fig:code_example}, the guidance can be more effective if we can leverage the value distance between \texttt{left\_bound} and \texttt{right\_bound} at the decision code branch at line 13.

    \item About \textit{planning failure discovery}: We clearly acknowledged that there are recent works able to discover semantic planning errors~\cite{fremont2020formal2}, and clarified that different from us, they (1) are designed for whole-system testing instead of planning-specific; (2) only consider overly-aggressive side, leaving the overly-conservative side unexplored; and (3) focus on safety instead of security (i.e., lack explicit threat model considerations).

    \item About \textit{geometric constraints}: We clearly acknowledged that the closest solution so far is from Scenic~\cite{fremont2019scenic}, which can generate test inputs within several generic geometric constraints in AD context (e.g., certain distances of a road object to curb). However, we also clarified that it still cannot address the more complicated ones specific to our problem context. For example, since we specifically want to generate road objects that should not affect the ego vehicle driving decision, their geometry constraints are inherently dependent on the planned trajectory of the ego vehicle, e.g., cannot be on or have any intention to move to any lanes that the ego vehicle plans to drive on (PI-C1, C4, C5 in Table~\ref{tab:phy_constraints}). However, Scenic's current design does not consider such dependencies.
    
    \item About \textit{Waymo example}: We clearly acknowledged that there is no official report on the root cause, so we cannot be certain that this is caused by planning flaws/bugs. We also clarified that we suspect that is likely the case as the environmental perception results (e.g., the detection and tracking of traffic cones and passing vehicles) are all correct according to the in-vehicle display~\cite{youtube_stuck_3}.
\end{itemize}
\end{response}

\begin{revision}\label{rev:overclaim}
We address the false claims on \textit{quantitative feedback} and \textit{geometric constraints} in the design challenge section (\S\rom{3}-B); those on \textit{planning failure discovery} at the beginning of the introduction (\S\rom{1}), and emphasize that our novelty is being the first specifically for \textit{overly-conservative} behavioral planning behaviors throughout the paper (e.g., in the abstract, introduction); and those on the \textit{Waymo example} in the last paragraph of \S\rom{2}-B ``Attack goal: Semantic Denial-of-Service (DoS) of BP''. 
%We tone down the claims in the first paragraph of \S\rom{1} and challenges in \S\rom{3} to avoid potential overclaims. 
\end{revision}

\textit{(3) Clarify whether making the design/implementation more aggressive or keeping it conservative and other possible ways to address issues that arise from conservative design.}

\begin{link}
\textbf{Corresponding original reviews:}

Reviewer A:

\textit{I personally think the planning module should keep conservative because the perception module might return errors, either natural or adversarial. Therefore, I think a more interesting direction for future work is to detect such attacks that exploit conservative designs. I hope the author could discuss more about this design dilemma in the paper.}
\end{link}

\begin{response}
We agree with Reviewer A that such overly-conservative designs cannot be trivially addressed by directly making the design/implementation more aggressive, since their fundamental causes are the non-trivial trade-off between safety and availability in AD context. For example, a direct idea to solve V1 and V8 is to reduce the safety buffer configuration to road-side static objects, but since such existing configurations may already be sufficiently tuned to ensure safety, changing them may compromise safety. One potential design direction for better addressing this trade-off is to consider dynamic configurations instead of fixed ones, e.g., dynamically adjusting the safety margin based on the velocity, since the required safety distance will decrease with smaller velocity~\cite{shalev2017formal} (which is one reason why highway lanes are wider than local ones~\cite{lane_width_speed_relationship}). However, how to design such dynamic adjustment is also non-trivial since various internal and external driving factors need to be systematically considered (e.g., internal ones such as vehicle size/speed, external ones such as the static/dynamic road conditions). We also agree attack detection is a promising direction for future work, e.g., detecting the placement patterns of road-side static obstacles for V1 and V8. 
%exploring the trade-off between safety and availability and how to detect DoS attacks is an interesting direction to explore in the future. We include a potential fix for each vulnerability in case studies and introduce more discussion.
\end{response}

\begin{revision}\label{rev:clarify_mitigation}
We clarified that such overly-conservative designs cannot be trivially addressed by directly making the design/implementation more aggressive in \S\rom{7}-A ``Solution discussions'', and also further clarified that this is due to the non-trivial trade-off between safety and availability in AD context. We also (1) discussed the potential design direction to better address this trade-off (dynamically adjusting the safety margin); and (2) pointed out that attack detection is a promising direction for future work.
%We add discussion on the potential fix of the discovered vulnerabilities in \S\rom{6}. We also point out the trade-off between safety and availability and list this as a promising future direction in \S\rom{7}-A.
\end{revision}

\textit{
(4) Provide capabilities of a stronger attacker that might also be able to compromise the perceptional sensors.}
\begin{link}
\textbf{Corresponding original reviews:}

Reviewer A:

\textit{Another weakness of the paper is the weak attack model where the attacker can only place physical objects. A stronger attacker might also be able to compromise the perceptional sensors, etc. as the authors themselves already pointed out. If a stronger attacker were assumed, more vulnerabilities might have been discovered. I understand the sufficiency of assuming a weak attacker as the first step on this research direction, but I would still suggest the authors discuss about this a bit more.}

\end{link}
\begin{response}
Thanks a lot for suggesting such threat model possibilities. To trigger the semantic DoS vulnerabilities in this paper, attackers may indeed also attack the perceptional sensors, such as by sensor spoofing~\cite{cao2019adversarial} or compromising internal AD system components~\cite{jha2020ml}, to introduce malicious inputs to BP similar to the physical-world attack vectors we considered (e.g., using sensor spoofing to inject fake road-side objects to perception outputs). In comparison, these attack vectors may have stronger BP input perturbation capabilities/flexibility, and thus more BP DoS vulnerabilities may indeed be discovered. However, we would also like to point out that that such attack vectors may also have a downside in that they may also introduce new attack requirements/costs, e.g., sensor spoofing equipment~\cite{cao2019adversarial} and access to internals or the supply chain of AD systems~\cite{jha2020ml}, which may make the exploitation of the discovered vulnerabilities less realistic/practical. Nevertheless, it is indeed an interesting direction (can lead to attacks with different properties) and we will clearly point this out in the paper.
%We thus decide to leave the exploration of such threat model direction to future work.
%We agree with the reviewer that this is an interesting problem. We want to point out that once the attacker can directly compromise the perceptional sensors, DoS attack is very straight forward since the attacker can directly inject a fake obstacle in front of the AD vehicle and force the AD vehicle to stop. This is an orthogonal attack approach since the attacker does not rely on the vulnerability in BP while she has to exploit vulnerabilities in sensors or perception algorithm to compromise the object detection results, which is out of our scope. We add more discussion on possible DoS attack approaches and point out that our focus is to exploit the BP DoS vulnerabilities. 
\end{response}
\begin{revision}\label{rev:stronger_threat_model}
We added a dedicated discussion on this threat model direction in `Stronger threat models'' at the end of \S\ref{sec:limitation}. We also mentioned this possibility in the threat model section (\S\ref{subsec:threat_model}).
%We include more discussion in the threat model section (Sec.~\ref{subsec:threat_model}) about other DoS attacks in AD systems, such as compromising the perceptional sensors. We also clarify that this is orthogonal to our work.
\end{revision}

\textit{(5) Defend/explain changing large safety margins and fine-tuning the related parameter values that would not compromise the safety requirements of ADs.}
\begin{link}
\textbf{Corresponding original reviews:}

Reviewer C:

\textit{The authors claim that the semantic DoS vulnerabilities discovered in this paper are caused by the large safety margins and suggest fine-tuning the related parameter values. However, such values may already be sufficiently tuned to ensure safety, so changing them may compromise safety. Authors should have shown that changing such values would not compromise safety requirements of ADs.}
\end{link}
\begin{response}
We agree with Reviewer C that our previously suggested fine-tuning solutions for the safety margins are flawed; just as pointed out by Reviewer C, since such existing configurations may already be sufficiently tuned to ensure safety, changing them may compromise safety. Fundamentally, such conservative designs are non-trivial to fix due to the challenging trade-off between safety and availability in AD context. 
%we should discuss the possibility of fixing the vulnerabilities. We want to point out that fixing such vulnerability is more complicated than just fine-tuning related parameters. The reason behind DoS vulnerabilities are more complicated than inappropriate parameter setup, such as program implementation error, failure to infer the intention of other objects, and failure to adjust the buffer dynamically based on environment and moving status of the ego vehicle. We explain potential fixes that would not compromise the safety while still keeps the availability under the vulnerable setups. We demonstrate that such overly-conservative planning behaviors are avoidable without compromising safety via a smarter planning design to validate the discovered vulnerabilities.
\end{response}

\begin{revision}\label{rev:tune_params}
We removed all previous discussions on the fine-tuning solution direction in \S\rom{7}-A, and clarified that such overly-conservative designs cannot be trivially solved by directly reducing the safety buffer configuration to road-side static objects. We also emphasized that such non-triviality is due to the challenging trade-off between safety and availability in AD context. 
%We add discussion about the potential fix for each discovered vulnerability in \S\rom{7}-A. We explain that fixing the problem is more complicated than just adjusting parameters and there do exist potential fixes which can guarantee the safety and availability at the same time for each vulnerability.
\end{revision}


\textit{(6) Defend/explain the need for BPFuzz over an approach that finds the ranges for placement of different physical objects that cause the vulnerabilities.}
\cut{
\begin{link}
\textbf{Corresponding original review:}

Reviewer B:

\textit{After reading the decision logic of behavior planning algorithms (Figure 2), the root cause of the DoS attacks introduced in the paper is due to the fact that the BP algorithms apply overly conservative decisions (lateral buffer (0.4m) for the detected objects) while computing the driving space. Here I fail to understand whether the goal of the BPFuzz is to find this particular bug or to find scenarios that trigger this bug in AD behavioral planning algorithms. If the paper claims to achieve the latter, the paper might give some concrete cases (positioning of different objects considering the vehicle size and environment it is operating) that cause the bugs, which might be a better approach than reporting a set of scenarios as vulnerabilities.}
\end{link}
}

\begin{response}
Thanks a lot for bringing up this possible design direction. At this point, similar to other dynamic testing approaches, our method can only provide several example triggering inputs (i.e., placements of the physical objects) for a discovered vulnerability, which is indeed less informative than an approach that can output the complete triggering ranges of such placements. However, we would like to first emphasize that we are not aware of any existing method/tool that can readily achieve that, at least for semantic BP DoS vulnerability. Thus, the lack of such exploration does not affect the value of our current effort, especially considering that we are the first to design such an automated discovery method for semantic BP DoS vulnerabilities. 

Second, we would like to point out that although there are possible solution strategies to achieve that, e.g., leveraging more sophisticated formal methods such as symbolic execution~\cite{cadar2008klee}, their application to our problem setting is far from trivial since (1) such methods are known to generally suffer from scalability limitations when applied to real-world code bases~\cite{ramos2015under}; and (2) in our problem settings one needs to further overcome the semantic gaps by systematically locating and extracting the physical object-related code-level constraints. We believe a systematical exploration of this worths a standalone future research work. 

%We think the idea of finding ranges for placements of different physical objects that cause the vulnerabilities is a brilliant idea. First, to the best of our knowledge, we are not aware of the existence of such a tool. We set our goal as to build a dynamic testing tool to discover a set of test cases representing the vulnerabilities since we even do not know the existence of vulnerabilities. Second, finding the range of placements will help the developers better understand the vulnerabilities and we consider this as a future direction. 
\end{response}

\begin{revision}\label{rev:find_range}
We add dedicated discussions on this potential design direction at the end of \S\rom{7}-B, ``Tool effectiveness'', and clearly pointed out the value of such a design direction and also its potential research challenges when explored in our problem setting. We also added more clarification about the system output at the end of \S\ref{sec:bpfuzz_design} ``System input/output and  assumptions''.
\end{revision}

\textit{(7) Provide the manual effort required in BPFuzz.}
\cut{
\begin{link}
\textbf{Corresponding original reviews:}

Reviewer B:

\textit{Required manual effort is not clear. Please detail the manual effort required in BPFuzz.}
\end{link}
}
\begin{response}
We agree with the reviewers that the manual effort is very important and is currently not very clear in the paper. Three types of manual efforts are required for using BPFuzz: (1) Collecting BP input traces for the targeted scenarios. Since BPFuzz is designed for AD developers, we assume that they can have direct access to such traces from their AD system testing or operations; (2) identifying PIs for the targeted scenarios. Note that such identification is an one-time effort and there are general ones applicable across multiple scenarios as identified later in~\S\ref{tab:summary_planning_invariant}; and (3) identifying and annotating the attack target positions in the source code. For AD systems developers, we assume that they can have high-level knowledge of the BP step (e.g., BP decision APIs and state variable class) to identify these based on the desired planning behavior of a PI and the state variables associated with the planning scenarios. In our experiments, it took less than 50 lines in total and less than 1 hour of manual efforts for an author who is experienced with the AD planning code.


%Two types of manual efforts are required: (1) Identify the PIs. Such task is a one-time effort and can be used across different AD software. (2) Identify and annotate the attack target positions in the source code. This only takes less than 1 hour of manual efforts for an experienced developer.
\end{response}

\begin{revision}\label{rev:manual_effort}
We added a dedicated description on this under ``Manual efforts'' in \S\rom{4}-B. 
%include the aforementioned discussion into \S\rom{7} Manual efforts.
\end{revision}

\textit{For related work, PC wants to see a clear discussion on the challenges of extending other fuzzers to discover BP DoS vulnerabilities.}
\begin{response}\label{rev:extend_fuzzer}
Thanks a lot for suggesting this important discussion. To extend traditional fuzzers to discover the semantic BP DoS vulnerabilities in this paper, they need to at least change the testing oracle from generic software symptoms (e.g., crashes) to the semantic ones (overly-conservative planning decisions). For the latter, a valid and systematic definition is the very first design challenge that needs to overcome (\S\ref{subsec:design_challenge}). However, that is still not enough since to achieve effective discovery they further need to add new problem-specific input generation and guidance designs such as those we designed (\S\ref{subsec:vuln_dist}, \ref{subsec:design_mutation}); otherwise, they still cannot discover any such vulnerabilities even given 24hr as concretely shown in~\S\ref{subsec:evaluation_ablation}. 
\end{response}
\begin{revision}
We added a dedicated discussion on this under ``Traditional fuzzers'' in the related work section (\S\rom{8}).
%We add a discussion on the challenges of extending other fuzzers to discover BP DoS vulnerabilities in \S\rom{7} Possibility of applying traditional fuzzer.
\end{revision}

\textit{
Address spelling and grammar issues throughout; you may consider the university editing services for assistance if they are available at your institution(s).}

\textit{Improve the organization and presentation of the paper.}
\begin{revision}
We are sorry about the spelling and grammar issues. We double-checked the paper multiple times and also asked a native speaker to help us in this, which was able to identify various new ones (quite some starting from \S\rom{2}) and have fixed them. We also tried our best to refine the organization and figures in the paper, especially those pointed out by the reviewers (e.g., clarity of Fig.~5 and location of Table II).
%invited our native collaborator to help us address grammar and spelling issues in the paper. Especially for Reviewer-A's question, we fix the sentence in the 3rd paragraph of \S\rom{1}.
\end{revision}

%\begin{revision}
%We would like to thank the reviewers for carefully reading the paper. We refine the organization and figures in the paper. Especially for comments from Reviewer-B, we change the original Fig.~5 to make it clear, and we move the original Table II to earlier page such that the readers can quickly find the result table. \tofix{Change the position of the table when we finish cutting.}
%\end{revision}
\textit{Clarify all points and make changes promised in your rebuttal.}
\begin{revision}
We delivered all promised clarification and changes in our rebuttal, for example evaluation improvements (Revision \ref{rev:trace_collection}, \ref{rev:evaluation_metric}), threat model explanations (Revision \ref{rev:exploit}, \ref{rev:case_exploitation}, \ref{rev:stronger_threat_model}), toning down overclaims (Revision \ref{rev:overclaim}), vulnerability definitions (Revision \ref{rev:distinction}), and trade-off between safety and availability (Revision \ref{rev:clarify_mitigation}, \ref{rev:tune_params}).

%We have clarified and made changes based on the major revision requirements list and original reviews. Please check our revision summary for more details. 
\end{revision}

\textit{The expectation in the revised design and evaluation sections is that your technique is not only understandable to the reader but can also be independently replicated by other researchers after reading your paper.}

\begin{revision}
Thanks a lot for emphasizing this. We tried our best to revise the design and evaluation sections to improve the clarity, especially those pointed out by the reviewers (Revision \ref{rev:evaluation_setup}, \ref{rev:test_goal}, \ref{rev:manual_effort}, \ref{rev:extend_fuzzer}). In addition, we will publicly release the BPFuzz source code and evaluation data upon paper acceptance to ensure reproducibility (indicated at the end of \S\rom{1}).

%We want to thank the reviewers for clarifying the requirements. We refine the writing in \S\rom{4} and \S\rom{5}. We will organize our implement and make it open-source later such that other researchers can easily reproduce our design and evaluation. We also add this promise in the last paragraph of \S\rom{1}.
\end{revision}

\textit{If any of these requirements are unclear, please use the anonymous comment system. We are looking forward to reviewing your revised submission.}

\begin{response}
We would like to sincerely thank the reviewers for offering such help. The provided revision requirements read clear enough to us so we directly performed revision based on those.
\end{response}

\cut{
\subsection{Responses to Other Review Comments}
\label{sec: other-comments}

%\alfred{please do this in a per-reviewer  fashion; see Ningfei's as an example}

In this section, we respond to several other issues raised in the individual reviews but not included in the list of required changes above.

\textbf{Reviewer B:}


\textit{I felt that the problem considered by the authors might be in the early stages of deployment for the current autonomous driving. Are these systems deployed in fully autonomous vehicles without any drivers or still at the testing stage in some specific cities? }

\begin{response}
We want to clarify that the AD companies have got deployment permits from government and have started to offer commercial service to the public even without safety drivers. Such examples have already been included in the \S\rom{2}-B Problem seriousness.
\end{response}



\textit{Additionally, I'm convinced that there is a disruption of service, but I am not fully convinced whether there is always a safety problem in all such cases and whether there is a human driver that can take action to address the disruption or the problem can be solved remotely.}

\begin{response}
We want to clarify that there exists possibility that DoS vulnerabilities can lead to safety problem instead of it can always cause safety problem.
\end{response}
\begin{revision}
We include the clarification into \S\rom{2}-B Problem seriousness.
\end{revision}




\textit{Real-world example in Figure 1 and motivating example in Figure 2 is not convincing.}



 \textit{Lastly, It is not clear from Figure 1 [63] the reason makes the car got stuck in the middle of the road and how authors are sure that this is due to Waymo's behavior planning algorithm as motivated in Figure 3. The authors would consider providing more evidence for this motivating example.}

\begin{response}
We want to clarify that we do not claim that the original Figure 1 is directly related to the original Figure 2 and 3. We want to use Figure 1 as a real world example to demonstrate that there exists a disruption of service for Waymo's AD vehicle. We can just say that this example is likely to be caused by planning's design flaws or bugs since the perception (the surrounding objects can be successfully detected) and control (the AD vehicle can drive automatically after getting rid of the stuck) components can work well in the video. 
\end{response}

\begin{revision}
We clarify that there is no direct relationship between Waymo's stuck example and the motivating example we discovered in the 3rd paragraph of \S\rom{2}-B.
\end{revision}


\vspace{0.8cm}
\textbf{Reviewer D:}

\textit{The format of the paper seems off. It is often very crowded and difficult to read. It definitively should not have passed the submission requirements.}
\begin{response}
We are sorry for the crowded space usage. 
\end{response}

\begin{revision}
We carefully reorganize the paper structure and make sure that our submission can pass the submission requirements. We pay extra attention to addressing the crowded space usage issue and make our paper easy to read.
\end{revision}

\vspace{0.8cm}
\textbf{Reviewer E:}

 \textit{I'd like to see some performance numbers which compare the effectiveness of the analysis phase and the simulation phase. How long do simulations take? What hardware was used?}
 


\begin{response}
We want to clarify that we do not include simulation in the testing process, since we directly give perception and prediction results as the test inputs.
\end{response}

\begin{revision}
%We have added the hardware used for testing in \S\rom{5} 

We have included the running time of each testing stage in Appendix K. We also clarify the inputs and outputs of BPFuzz and testing in \S\rom{5} Test input generation.
\end{revision}
}
